Large totally symmetric sets

A totally symmetric set is a subset of a group such that every permutation of the subset can be realized by conjugation in the group. The (non-)existence of large totally symmetric sets obstruct homomorphisms, so bounds on the sizes of totally symmetric sets are of particular use. In this paper, we prove that if a group has a totally symmetric set of size $k$, it must have order at least $(k+1)!$. We also show that with three exceptions, $\{(1 \; i)\mid i = 2,\ldots,n\} \subset S_n$ is the only totally symmetric set making this bound sharp; it is thus the largest totally symmetric set relative to the size of the ambient group.

==> Scraps.tex <==
The proof is essentially a counting argument via the orbit stabilizer theorem. Let $X$ be a totally symmetric set of cardinality $k$, and consider the action of $G$ on totally symmetric sets by conjugation. Because $X$ is totally symmetric, the natural map $\Stab(X) \to S_X\cong S_k$ is a surjection, meaning $|\Stab(X)|\geq k!$. It remains to show $|\Orb(X)|\geq k+1$. 

We first deal with the worst-case scenario, where $\Orb(X) = 1$. This forces $X$ to be an entire conjugacy class---if $x\in X$ but $gxg\inv \not \in X$, then $gXg\inv \in \Orb(X)$.    

\begin{lemma}
Let $G$ be a group and $X$ a non-commutative totally symmetric set of cardinality $k$. If $X$ is an entire conjugacy class, then $k \leq 3$.
\end{lemma}

\begin{proof}
do it...
\end{proof}


Now that we are guaranteed conjugates $Y \in \Orb(X)$ distinct from $X$, we may additionally hope that $Y \cap X$ is non-empty. This is desirable, since the total symmetry of $X$ allows us to produce more elements of its orbit---for any subset $P \subset X$ of cardinality $|P| = |Y \cap X|$, there is some $\sigma_P \in G$ such that $\sigma_P X \sigma_P\inv = X$ and $\sigma_P (Y \cap X) \sigma_P = P$. The totally symmetric sets $Y_P \coloneqq \sigma_P Y \sigma_P\inv$ are distinct, as they have different intersections with $X$. There are at least $k$ such totally symmetric sets $Y_P$, which (together with $X$) show $|\Orb(X)| \geq k+1$, completing the proof in this case.

We proceed assuming any two distinct conjugates of $X$ are disjoint. In particular, any $x \in X$ fixes $X$ by conjugation, as $x \in x X x\inv$. Then $X \subset \Stab(X)$, meaning $X$ is totally symmetric in $\Stab(X)$. By definition of $\Stab(X)$, the conjugacy class of $x \in X$ in $\Stab(X)$ is exactly $X$, 




-------------------------

\begin{lemma}
The following facts are contradictory.  

\begin{enumerate}
    \item $X\subset H$ is totally symmetric in a group $H$.
    \item $k > 3$ (a hypothesis of \Cref{thm:main})
    \item Elements of $X$ do not pairwise commute
    \item $X$ is an entire conjugacy class of $G$.  
\end{enumerate}

\end{lemma}



% \begin{enumerate}
%     \item $X\subset \Stab()$ is totally symmetric in a group $H$ of cardinality $k$.
%     \item $k > 3$ (a hypothesis of \Cref{thm:main})
%     \item The elements of $X$ do not pairwise commute
%     \item $X$ is an entire conjugacy class of $G$.  
% \end{enumerate}

% \begin{lemma}
% \label{contradiction}
% Let $X \subset H$ be a non-commutative totally symmetric set of $H$ with cardinality $k$. If $X$ is an entire conjugacy class of $H$, then $k \leq 3$.
% \end{lemma}

% \begin{lemma}
% The following facts are contradictory.  

% \begin{enumerate}
%     \item $X\subset H$ is totally symmetric in a group $H$.
%     \item $k > 3$ (a hypothesis of \Cref{thm:main})
%     \item Elements of $X$ do not pairwise commute
%     \item $X$ is an entire conjugacy class of $G$.  
% \end{enumerate}

% \end{lemma}

% \begin{proof}
% \todo[inline]{Do it.}
% \end{proof}



From the proof of part 1, we know $|\Orb(X)| = k+1$, and moreover that there is some $Y \in \Orb(X)$ for which $\Orb(X) = \{\}$ intersects $X$ non-trivially. As $\binom{k}{||}$ This intersection $X \cap Y$ must either contain a  



-----------------

\todo[inline]{I've decided to dramatically cut down the corollary.}


As a sample application of \Cref{thm:classification}, we use this result to give a short, conceptually simple proof of the well-known classification of homomorphisms $S_n \to S_m$ for $n \geq m$ due to Hölder \cite{Holder}. The basic idea is that \Cref{thm:classification} determines all possible images of $f(X_n)$. 


\begin{corollary}[Hölder]
\label{corr}
Let $n \geq m > 2$ and $f:S_n \to S_m$ be a homomorphism. Then

\begin{enumerate}
     \item If $n > m$ and $(n,m) \neq (4,3)$, then $\Image(f)$ is cyclic.  
    \item If $n = m \neq 6$ and $\Image(f)$ is non-cyclic, then $f$ is an inner automorphism.
    \item \label{out} If $n = m = 6$ and $\Image(f)$ is non-cyclic, then $f$ is an automorphism. Furthermore, $\Out(S_6) \cong \Z /2\Z$.
    \item If $(n,m) = (4,3)$ and $\Image(f)$ is non-cyclic, then $f$ is conjugate to the exceptional map $g: S_4 \to S_3$ defined by $g(1 \: 4) = (1 \: 2)$, $g(2 \: 4) = (1 \: 3)$ and $g(3 \: 4) = (2 \: 3)$.
\end{enumerate}




------------------

This is before I gutted the proof of corollary 3.

--------------------

We break this up into three cases: 

\begin{enumerate}
    \item  $n \not \in \{3,4,6\}$ and $n = m$
    \item $n = m = 6$
    \item $ (n,m) = (4,3)$
\end{enumerate}



\vspace{.2cm}

\noindent \textit{Case 1:} $n \not \in \{3,4,6\}$ and $n = m$. By Theorem \ref{thm:classification}, there is some $\sigma \in S_n$ so that $f(X_n) = \tilde{\sigma} (X_n)$, where $\tilde{\sigma}$ is the inner automorphism corresponding to $\sigma$. Then $(\tilde{\sigma}\inv \circ f)(X_n) = X_n$, that is $\tilde{\sigma}\inv \circ f$ permutes $X_n$. Total symmetry now gives an element $\tau \in S_n$ realizing this permutation so that $\tilde{\tau}\inv \circ \tilde{\sigma}\inv \circ f$ is the identity map on $X_n$. Then $f = \widetilde{\sigma \tau}$ is an inner automorphism as desired.

\vspace{.2cm}

\noindent \textit{Case 2:} $n = m = 6$. If $f(X_n)$ is conjugate to $X_n$, then $f$ is an inner automorphism by the previous paragraph. By Theorem \ref{thm:classification},  $f(X_n)$ may additionally be conjugate to $\rho(X_n)$, where $\rho$ is the outer automorphism given in Section \ref{proof}. In this case, $(\rho\inv \circ f) (X_n)$ is conjugate to $X_n$, meaning $(\rho\inv \circ f)$ is an inner automorphism. In particular, $f$ is an automorphism and $[\rho] = [f]$ in $\Out(S_n)$.
\vspace{.2cm}

\noindent \textit{Case 3: $(n,m) = (4,3)$.} Because $\Image(f)$ is non-cyclic, $f(X_n)$ is a totally symmetric set of cardinality $3$ in $S_3$. By Theorem \ref{thm:classification}, there is only one such totally symmetric set: $\{(1 \: 2), (1\: 3), (2\: 3)\}$. Then $f(1 \: 4) = (1 \: 2)$, $f(2 \: 4) = (1 \: 3)$ and $f(3 \: 4) = (2 \: 3)$, up to possibly permuting the right sides of these equalities. Any such permutation can be realized by conjugation, so $f$ is conjugate to the exceptional map $g:S_4 \to S_3$, as desired.



---------------------

Before I re-arranged

\note{give more of a road map}

Let $X$ be a totally symmetric set of cardinality $k$ in a group $G$. The proof of \Cref{thm:main} is essentially an orbit-stabilizer argument applied to the action of conjugation on totally symmetric sets. By total symmetry, the natural map $\phi:\Stab(X) \to S_k$ is surjective, and therefore $|\Stab(X)| \geq k!$. It remains to show $|\Orb(X)| \geq k+1$. 

If any $Y \in \Orb(X)$ intersects $X$ non-trivially, we can use total symmetry to produce $\binom{k}{|X \cap Y|} \geq k$ other elements of $\Orb(X)$ as follows. For each $|X\cap Y|$-element subset $A \subset X$, let $g_A \in \Stab(X)$ be such that $g_A(X \cap Y)g_A\inv = A$. Then the $g_AYg_A\inv$ are all distinct, as they have different intersections with $X$. This proves $|G|\geq (k+1)!$ in this case.

We proceed assuming any two distinct totally symmetric sets conjugate to $X$ are disjoint. In particular, any $a \in X$ satisfies $aXa\inv = X$, meaning $X \subset \Stab(X)$ is a totally symmetric set in $\Stab(X)$. Moreover, $X$ is an entire conjugacy class of $\Stab(X)$. If any $a \in X$ satisfies $\phi(a) = e$, then the elements of $X$ pairwise commute, and we may apply \cite[Proposition 2.2]{Finite_Quotients} to obtain the bound $|G| \geq k!\cdot 2^{k-1}$. 

We additionally assume $\phi(X) \neq \{e\}$. Because $\phi:\Stab(X) \to S_k$ is surjective, $\phi(X)$ is also an entire conjugacy class of $S_k$ consisting of elements fixing at least one point. For $k > 3$, such conjugacy classes in $S_k$ have cardinality larger than $k$. This contradicts $|X| = k$, and completes the proof that $|G|\geq (k+1)!$.

\vspace{.3cm}
\end{corollary}
